Predictive Monitoring of Black-Box Dynamical Systems

We study the problem of predictive runtime monitoring of black-box dynamical systems with quantitative safety properties. The black-box setting stipulates that the exact semantics of the dynamical system and the controller are unknown, and that we are only able to observe the state of the controlled (aka, closed-loop) system at finitely many time points. We present a novel framework for predicting future states of the system based on the states observed in the past. The numbers of past states and of predicted future states are parameters provided by the user. Our method is based on a combination of Taylor's expansion and the backward difference operator for numerical differentiation. We also derive an upper bound on the prediction error under the assumption that the system dynamics and the controller are smooth. The predicted states are then used to predict safety violations ahead in time. Our experiments demonstrate practical applicability of our method for complex black-box systems, showing that it is computationally lightweight and yet significantly more accurate than the state-of-the-art predictive safety monitoring techniques.

==> experimentsf1tenth.tex <==


We evaluate our method on a set of experiments in the F1Tenth environment, considering a total of three different metrics for the performance of our method vs. the baseline TTC method. First, we collect a total of 3.500.000 timesteps from the F1Tenth simulator with a total of 70 differently parametrized Follow the Gap \cite{} and Pure Pursuit \cite{} agents. \color{blue}[I took these agents from my master thesis] \color{black}. We consider a total of 16 Follow the Gap Agents and 54 Pure Pursuit agents. Each agent is rolled out from a random starting point for a maximum of 1000 steps per episode. We then remove a set amount of initial timesteps as the monitor does not provide predictions for some number $p$ (I set the initial cutoff to 20, which is actually to much for our current methods, as they all start producing values at $<t=4$, however, if we add some other method that needs less than 20 steps to initialize I can easily add it without rerunning everything). We also remove episodes that are to short, leaving us with between 49,050 and 45,896 timesteps per agent in our dataset.

Based on this dataset we compute the predictions with TTC and the Static method for each episode. Below the results and metrics we consider are presented.

\textbf{Euclidean distance error}: The Euclidean distance error measures the difference between the actual and predicted states in terms of their spatial positions. The results, shown in Figure~\ref{fig:f1tenth mse}, are plotted as a function of the lookahead distance, focusing only on the x and y coordinates. \color{blue} It might be that the agents dont just differ because of the reduced smoothness of FTG, but also that it might be that FTG agents are on average faster (I have not checked this)\color{black}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/euclidean_group_subplots_side_by_side.pdf}
    \caption{Euclidean distance error for TTC and Static methods, showing the two categories of agents we consider.}
    \label{fig:f1tenth mse}
\end{figure}

\begin{comment}
\begin{table}[ht]

	\centering
	\caption{Performance Comparison of TTC, ARIVA and Static Methods}
	\label{tab:performance_comparison_f1tenth}
	\begin{tabular}{lcccccccccc}
		\toprule
		\multirow{2}{*}{\textbf{Env}} & 
		\multicolumn{4}{c}{\textbf{TTC Method}} & 
		\multicolumn{4}{c}{\textbf{ARIVA Method}} & 
		\multirow{2}{*}{\textbf{Safety Rate}} \\
		\cmidrule(lr){2-5} \cmidrule(lr){6-9}
		& TP & NP & FP & quanti.  & TP & NP & FP & quanti.  & & \\
		\midrule
		F1Tenth &  &  &  &  &  &  & & &  \\
		% Add more benchmark rows as needed
		\bottomrule
	\end{tabular}
\end{table}
\end{comment}
\textbf{Boolean Safety Metric:} This metric evaluates the minimum distance to a wall, set at $d=0.5$ meters. Results for the FTG and Pure Pursuit methods are presented in Table~\ref{tab:performance_comparison_boolean}. A true positive (TP) is recorded when an unsafe state is accurately predicted between 30 and 50 timesteps before it occurs. \color{red} [I do not check if this warning is actually in n steps, but rather I reduce the prediction array (1-50) to a single number, taking the minimum. Hence, if 30-50 steps before there is any warning in the prediction array I record a TP. this warning could for instance also be predicting a crash in 10 steps.]\color{black} A false negative (FN) occurs if no prediction is made within this timeframe before an unsafe state, while a false positive (FP) is recorded if an unsafe state is predicted but does not occur within the next 50 timesteps.





\begin{table}[h!]
	\centering
	\caption{True Positive, False Positive, and False Negative Comparison for FTG (775300 timesteps) and Pure Pursuit (2647570 timesteps).}
	\label{tab:performance_comparison}
	\begin{tabular}{lcccccc}
		\toprule
		\textbf{Method} & \multicolumn{3}{c}{\textbf{FTGAgent}} & \multicolumn{3}{c}{\textbf{Pure Pursuit}} \\
		\cmidrule(lr){2-4} \cmidrule(lr){5-7}
		& \textbf{TP} & \textbf{FP} & \textbf{FN} & \textbf{TP} & \textbf{FP} & \textbf{FN} \\
		\midrule
	Static & 106281 & 36329 & 2889 & 255376 & 33049 & 628 \\ 
	Ttc & 80187 & 12371 & 28983 & 236694 & 100915 & 19310 \\ 
		\bottomrule
	\end{tabular}
	\end{table}
	
	
\begin{table}[h!]
	\centering
	\begin{tabular}{|l|l|r|r|r|r|r|}
	\hline
	\textbf{Agent Group} & \textbf{Method Name} & \textbf{TP (\%)} & \textbf{FP (\%)} & \textbf{FN (\%)} & \textbf{Length} & \textbf{Mean Warning Time} \\ \hline
	FTG & static & 98736 (12.74\%) & 177354 (22.88\%) & 298 (0.04\%) & 775300 & 98.09 ± 5.92 \\ \hline
	FTG & ttc & 90232 (11.64\%) & 133671 (17.24\%) & 8802 (1.14\%) & 775300 & 90.93 ± 21.17 \\ \hline
	pure_pursuit & static & 244257 (9.23\%) & 238744 (9.02\%) & 2155 (0.08\%) & 2647570 & 96.67 ± 9.47 \\ \hline
	pure_pursuit & ttc & 214305 (8.09\%) & 566401 (21.39\%) & 32107 (1.21\%) & 2647570 & 84.38 ± 23.29 \\ \hline
	
	\end{tabular}
	\caption{Performance metrics grouped by agent group and method name, with percentages relative to the total length and mean warning time.}
	\label{tab:agent_metrics}
\end{table}
	


\textbf{Early Warning Metric:} This metric assesses the system's ability to predict unsafe states using a lookahead window of 100 timesteps. Results for the FTG and Pure Pursuit methods are presented in Table~\ref{tab:performance_comparison}. The metric calculates the earliest time before an unsafe state where a warning is issued. A true positive (TP) is recorded if a warning is correctly generated within the 100-timestep window prior to an unsafe state. A false negative (FN) occurs if no warning is issued before the unsafe state, while a false positive (FP) is recorded if a warning is issued, but no unsafe state occurs within the lookahead window. \color{red} [I do not check if this warning is actually in n steps, but rather I reduce the prediction array (1-100) to a single number, taking the minimum. Therefore the algorithm looks like this: prediction array is initally of shape (N,100), where N is the number of timesteps. I reduce it to (N,) containing true and false, by taking the minimum across axis=1 and then checking the distance $d<0.5$]\color{black}




\begin{table}[h!]
	\centering
	\caption{Mean and Standard Deviation Comparison for FTG and Pure Pursuit.}
	\label{tab:performance_comparison}
	\begin{tabular}{lcccccc}
		\toprule
		\textbf{Method} & \multicolumn{3}{c}{\textbf{FTGAgent}} & \multicolumn{3}{c}{\textbf{Pure Pursuit}} \\
		\cmidrule(lr){2-4} \cmidrule(lr){5-7}
		& \textbf{Mean} & \textbf{Std} & \textbf{FP} & \textbf{Mean} & \textbf{Std} & \textbf{FP} \\
		\midrule
	Static & 98.09 & 5.92 & 106489 & 96.67 & 9.47 & 138326 \\ 
	TTC & 90.93 & 21.17 & 48336 & 84.38 & 23.29 & 297460 \\ 
	
		\bottomrule
	\end{tabular}
	\end{table}
	
	
	
\begin{comment}
The total length is less as I droped all that had no unsafe states. (but the FP still consider that, as i added it at the end for the above table)
		DataFrame for early warning metric:
   | agent_group   | method_name   |   combined_mean_warning_time |   combined_std_warning_time |   total_warnings |   total_FP |     total_length |
   |:--------------|:--------------|-----------------------------:|----------------------------:|-----------------:|-----------:|-----------------:|
   | FTG           | static        |                      98.0924 |                     5.92258 |            99034 |     106489 | 571495           |
   | FTG           | ttc           |                      90.9294 |                    21.1737  |            99034 |      48336 | 571495           |
   | pure_pursuit  | static        |                      96.6728 |                     9.47212 |           246412 |     138326 |      1.79838e+06 |
   | pure_pursuit  | ttc           |                      84.3781 |                    23.2891  |           246412 |     297460 |      1.79838e+06 
\end{comment}
   
